GenDICE: Generalized Offline Estimation of Stationary Values

An important problem that arises in reinforcement learning and Monte Carlo methods is estimating quantities defined by the stationary distribution of a Markov chain. In many real-world applications, access to the underlying transition operator is limited to a fixed set of data that has already been collected, without additional interaction with the environment being available. We show that consistent estimation remains possible in this challenging scenario, and that effective estimation can still be achieved in important applications. Our approach is based on estimating a ratio that corrects for the discrepancy between the stationary and empirical distributions, derived from fundamental properties of the stationary distribution, and exploiting constraint reformulations based on variational divergence minimization. The resulting algorithm, GenDICE, is straightforward and effective. We prove its consistency under general conditions, provide an error analysis, and demonstrate strong empirical performance on benchmark problems, including off-line PageRank and off-policy policy evaluation.

==> algbox.tex <==
%!TEX root = dual_ratio.tex

% \section{Algorithm Details}

\begin{algorithm}[H]
   \caption{GenDICE (with function approximators)}\label{alg:gendice}
\begin{algorithmic}
   \STATE {\bf Inputs}: Convex function $\phi$ and its Fenchel conjugate $\phi^*$, off-policy data $\Dcal = \{(s^{(i)}, a^{(i)}, r^{(i)}, s^{\prime(i)})\}_{i=1}^N$, initial state $s_0\sim\mu_0$, target policy $\pi$, {distribution corrector}~$\texttt{nn}_{\theta_\tau}(\cdot,\cdot), \texttt{nn}_{\theta_f}(\cdot,\cdot)$, constraint scalar $u$,  learning rates $\eta_\tau, \eta_f, \eta_u$, number of iterations $K$,
   batch size $B$.
   \FOR{$t = 1,\dots,K$}
   \STATE Sample batch $\{(s^{(i)}, a^{(i)}, r^{(i)}, s^{\prime(i)})\}_{i=1}^B$ from $\Dset$. 
   \STATE Sample batch $\{s_0^{(i)}\}_{i=1}^B$ from $\mu_0$.
   \STATE Sample actions $a^{\prime(i)}\sim\pi(s^{\prime(i)})$, for $i=1,\dots,B$.
   \STATE Sample actions $a_0^{(i)}\sim\pi(s_0^{(i)})$, for $i=1,\dots,B$.
   \STATE Compute empirical loss $\hat J_{\chi^2}\rbr{\tau, u, f} = \rbr{1 - \gamma}\EE_{\mu_0\pi}\sbr{f\rbr{s, a}} + \gamma\EE_{\Tcal_p}\sbr{\tau\rbr{s, a}f\rbr{s', a'}}$ \\
   $- \EE_{p}\sbr{\tau\rbr{s, a}\rbr{f\rbr{s, a} + \frac{1}{4}f^2\rbr{s, a}}} + \lambda\rbr{\EE_p\sbr{u\tau\rbr{s, a}-u}-\frac{u^2}{2}}$.
   \STATE Update $w_\tau\leftarrow \theta_\tau - \eta_\tau \nabla_{\theta_\tau}\hat J_{\chi^2}$.
   \STATE Update $w_f\leftarrow \theta_f + \eta_f \nabla_{\theta_f}\hat J_{\chi^2}$.
   \STATE Update $u\leftarrow \theta_u + \eta_u \nabla_{u} \hat J_{\chi^2}$.
   % \Bo{In the proof, I only have guarantees for optimization error from SVRG results. The vanilla SGD result is not known yet. But I think it is possible to derive.}
   \ENDFOR 
   \STATE {\bf Return} $\texttt{nn}_{\tau}$.
\end{algorithmic}
\end{algorithm}
